Sticker820K: Empowering Interactive Retrieval with Stickers

Stickers have become a ubiquitous part of modern-day communication, conveying complex emotions through visual imagery. To facilitate the development of more powerful algorithms for analyzing stickers, we propose a large-scale Chinese sticker dataset, namely Sticker820K, which consists of 820k image-text pairs. Each sticker has rich and high-quality textual annotations, including descriptions, optical characters, emotional labels, and style classifications. Although vision-language tasks in the domain of natural images have been well studied, directly applying the those models, such as CLIP, to sticker data is not an optimal solution due to the discrepant nature between natural and emotive image data. Therefore, we propose StickerCLIP as a benchmark model on the Sticker820K dataset. For the text-to-image retrieval task, our StickerCLIP demonstrates strong superiority over the CLIP, which achieves an absolute gain of 66.0\% in mean recall on the Sticker820K test set. Additionally, we endeavor to extend the recently popularized LLM by means of prompt tuning, integrating its ability for sticker retrieval and allowing users to retrieve stickers through instructions. We validate the feasibility of this method, demonstrating the immense potential of prompt tuning in expanding LLM abilities while not affecting the quality of upstream tasks.

==> 4-methodology.tex <==
\section{Methodology}

\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{StickerOverview.pdf}
  \caption{Overview of framework.}
  \label{fig:two_column_image}
\end{figure*}

In this paper, we employ comparative learning to align the visual and textual features of emoticons. We propose two benchmarks, namely: 1) StickerCLIP, in which we fine-tune the pre-trained CLIP model on sticker dataset, and 2) StickerLLM, in which we leverage the recent and popular LLM model and achieve prompt tuning to enable it to automatically extract semantic information related to stickers in user instruction while aligning with visual features without affecting LLM's performance on upstream tasks.

\subsection{StickerCLIP}
CLIP comprises a visual encoder $E_{\theta}$ and a text encoder $E_{\phi}$. Given a caption $T$ and its paired image $I$,  $E_{\theta}(I) \in \mathbb{R}^{d}$ and $E_{\phi}(T) \in \mathbb{R}^{d}$ represent the outputs of the visual encoder and text encoder, respectively. 
In order to align the text and visual features, CLIP employs InfoNCE loss \cite{oord2018representation} for text-to-image(t2i) and image-to-text(i2t) retrieval over a batch of N image-text pairs $(T_i,I_i)$, which can be formulated as follows:
\begin{align}
\mathcal{L}_{\mathrm{t} 2 \mathrm{i}} & =-\frac{1}{N} \sum_{i=1}^N\left(\log \frac{\exp \left(\operatorname{sim}\left(T_i, I_i\right) / \tau\right)}{\sum_{j=1}^N \exp \left(\operatorname{sim}\left(T_i, I_j\right) / \tau\right)}\right) \label{func:info_nce_t2i}\\
\mathcal{L}_{\mathrm{i} 2 \mathrm{t}} & =-\frac{1}{N} \sum_{i=1}^N\left(\log \frac{\exp \left(\operatorname{sim}\left(I_i, T_i\right) / \tau\right)}{\sum_{j=1}^N \exp \left(\operatorname{sim}\left(I_i, T_j\right) / \tau\right)}\right) \label{func:info_nce_i2t}
\end{align}
In the above formula, $\operatorname{sim}(I,T)$ represents the cosine similarity between the feature vectors of the image and the caption. $\tau$ is a learnable temperature parameter. The total loss is:
\begin{equation}
    \mathcal{L}_{total} = \mathcal{L}_{\mathrm{t} 2 \mathrm{i}} + \mathcal{L}_{\mathrm{i} 2 \mathrm{t}}
\end{equation}
In this paper, we employ ChineseCLIP \cite{yang2022chinese} and QA-CLIP as our pre-trained models. We concatenate different type of textual information and use it as input for the text encoder. Since the stickers we collected not only include static images, such as JPG and PNG, but also animated images, such as GIF, while the pre-trained CLIP model only takes static images as input. Therefore, we extract multiple frames of an animated image as input for the visual encoder and calculate the average vector along different frames. In the practice, we extract the first frame, the middle frame, and the last frame separately.

\subsection{StickerLLM}
Recently, LLM has garnered widespread attention and undergone intensive research due to its powerful text processing capabilities. Researchers have aligned LLM with human intent via instruction tuning and equipped it with the ability to utilize tools through prompt engineering. Furthermore, through expanding frozen LLM, researchers have enabled it to process multimodal information. 

In this paper, we further explore the potential to expand the capabilities of LLM with the goal of enabling it to retrieve stickers without disrupting upstream tasks. To achieve this objective, we added new tokens to LLM as representations of the tools. During the training process, we froze the majority of the parameters in LLM and only fine-tuned the weight parameters corresponding to the position of the new tokens in the token embeddings and logistic head.


As illustrated in Figure 2, StickerLLM comprises an LLM and a visual encoder. To effectively extract visual embedding from stickers, we obtain the visual encoder from finetuned StickerCLIP and freeze all its parameters. The LLM not only generates textual responses through auto-regressive modeling, but is also utilized for extracting text retrieval embedding. We introduce the <ret> token for this purpose.

To enable StickerLLM to retrieve stickers by following human instructions, the framework need to learn two objectives: 1) generating the text responese and <ret> token at an appropriate position based on contextual clues, and 2) empowering the <ret>  token with the ability to retrieve stickers.

The first objective can be achieved by maximizing the log likelihood of the token sequence, the loss can be factored as a sum of conditional log probabilities:
\begin{equation}
\mathcal{L}_{c}=\sum_{t=1}^t \log p_\theta\left(s_t \mid s_1, \ldots, s_{t-1}\right)
\end{equation}
where $p_\theta$ is the autoregressive LLM and $(s_1, \dots, s_T)$ is the sequence of input tokens. 

To achieve the second objective, we align the LLM's retrieval embedding with visual embedding by contrastive learning. We use a learnable linear layer $\mathbf{W}_t \in \mathbb{R}^{D \times d}$ to map the last hidden state of <ret> as the $h_{\theta}(s_i)^{T} \mathbf{W}_t \in \mathbb{R}^{d}$, where $h_{\theta}$ is the LLM without logistic head. The contrastive loss is the same with Eq. \ref{func:info_nce_i2t} and Eq. \ref{func:info_nce_t2i}. The total loss can be written as:
\begin{equation}
    \mathcal{L} = \mathcal{L}_c + \lambda (\mathcal{L}_{\mathrm{t2i}} + \mathcal{L}_{\mathrm{i2t}})
\end{equation}
$\lambda$ is the scale of contrative loss. 

To achieve the collaborative search using image and text, we endeavored to extract unified retrieval embeddings of visual and textual data through <ret>. If image is inputted, we initially extract the visual features through the frozen visual encoder of StickerCLIP. Subsequently, we map the aforementioned visual features onto the input of LLM by utilizing a learnable linear layer $\mathcal{W}_c \in \mathbb{R}^{d\times D}$.

Since the visual encoder and LLM is frozen, only the linear layer $\mathbf{W}_t$, $\mathbf{W}_c$, and the weight parameters corresponding to the position of the <ret> in the token embeddings and logistic head receive gradient updates.




==> 5-experiments.tex <==
\section{Experiments}

\subsection{Implementation Details}
Comparative experiments were conducted on StickerCLIP and StickerLLM. In StickerCLIP, the batch size equates to 2,048, the learning rate to 2e-5, and the weight decay to 1e-2. We employ the AdamW optimizer in tandem with a Cosine learning rate schedule, designate the content length of the text encoder as 64, and due to the potential inclusion of animated images, we extract features from the first, middle, and last frames as input for the visual encoder, subsequently averaging these features. In StickerLLM, the batch size is setting to 288 due to the limited memory, the learning rate and weight decay are setting to 2e-5 and 0. We also employ the AdamW optimizer in tandem with a Cosine learning rate schedule. we construct a single-round retrieval dialogue comprising question templates and response templates, with queries entailing user retrieval instructions and corresponding responses incorporating special tokens for retrieval. We implement chatGLM-6b as the language model in StickerLLM, introducing new special tokens such as <ret>, </ret>, <img>, </img>, and <pret>, the roles of which are outlined in the accompanying table. With a 50\% probability, we add <pret> to the beginning of the training data as prefix tuning to modulate generated probability distributions. Our StickerLLM is configured to accept both text and image inputs, facilitating text-to-image retrieval, image-to-image retrieval, and unified image-text-to-image retrieval. During data construction, we generate text-to-image retrieval data with a 50\% likelihood, image-to-image retrieval data with a 25\% probability, and since precise joint retrieval data pairing cannot be directly generated, we randomly extract images from the dataset with a 25\% probability to create image-text-to-image retrieval data, ensuring that the LLM attends to user input text when images are provided. This is exemplified in training data illustration 2. The last hidden state of the <ret> token is fed into a learnable, fully-connected layer to extract retrieval feature vectors.

\begin{table*}[t]
\centering

\setlength\tabcolsep{10pt}
\begin{tabular}{llcccccccc} 
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{4}{c}{Image-to-Text Retrieval} & \multicolumn{4}{c}{Text-to-Image Retrieval}  \\ 
\cline{3-10}
\multicolumn{1}{c}{}                       & \multicolumn{1}{c}{}                        & R@1  & R@5  & R@10 & MR                     & R@1  & R@5  & R@10 & MR                      \\ 
\hline
\multirow{3}{*}{RN50}                      & Zero-shot                                   & 5.8  & 12.8 & 17.0 & 11.9                   & 3.4  & 7.6  & 10.3 & 7.1                     \\
                                           & Freeze-vision                               & 43.3 & 61   & 66.5 & 56.9                   & 33.0 & 52.3 & 59.3 & 48.2                    \\
                                           & StickerCLIP                                 & 59.0 & 76.0 & 80.3 & 71.8                   & 57.9 & 75.4 & 79.8 & 71.0                    \\
\multirow{3}{*}{ViT-B}                     & Zero-shot                                   & 13.3 & 25.8 & 32.1 & 23.8                   & 8.8  & 18.1 & 23.0 & 16.7                    \\
                                           & Freeze-vision                               & 58.8 & 77.1 & 81.9 & 72.6                   & 52.4 & 72.9 & 78.5 & 67.9                    \\
                                           & StickerCLIP                                 & 71.4 & 87.7 & 91.2 & 83.4                   & 71.3 & 86.9 & 90   & 82.7                    \\
\bottomrule
\end{tabular}
\caption{Experimental results of various methods in text-to-image retrieval and image-to-text retrieval.}
\label{tab:sticker_clip_eval}
\end{table*}

\subsection{Performance of StickerCLIP}
We conducted experiments on two distinct model sizes, RN50 and ViT-B, comparing the following three methods: 1) Zero-shot, where we evaluated the pre-trained ChineseCLIP; 2) Frozen-vision, in which we froze the visual encoder within the CLIP and fine-tuned it on the Emoji820K training set; and 3) StickerCLIP, which involved fine-tuning all parameters on the Emoji820K training set. We assessed the performance on the Emoji820K test set and reported Recall@K (recall of the top K candidates) with K values of 1, 5, 10, and the Mean Recall (MR) for both image-to-text and text-to-image retrieval.

Tab. \ref{tab:sticker_clip_eval} displays the performance of various models and methods on the test set. Generally speaking, StickerCLIP outperforms the other two methods, achieving the best overall performance. For instance, in the ViT-B model, StickerCLIP exhibits a 59.6\% and 66.0\% improvement respectively over Zero-shot in the Mean Recall (MR) metric for Image-to-Text Retrieval and Text-to-Image Retrieval, and a 10.8\% and 14.8\% increase respectively in comparison to Frozen-vision. The inferior zero-shot performance of CLIP on StickerCLIP suggests that the sticker dataset exhibits significant differences in data features compared to the natural image-text pairs used for pre-training. Specifically, on the visual side, the Emoji820K dataset contains numerous hand-drawn images, such as cartoons, while on the textual side, Emoji820K encompasses a rich assortment of emotive vocabulary. Consequently, a considerable performance gap persists between StickerCLIP and models that fine-tune the text encoder only.

\subsection{Performance of StickerLLM}
The performance of StickerLLM can be divided into two aspects: (1) the ability to use retrieval tools in the correct context, that is, LLM should only produce responses containing the <ret> token when the user presents instructions related to retrieving stickers. (2) The retrieval performance of the <ret> token in the retrieval task. We designed the following experiments to evaluate StickerLLM.

\textbf{Accuracy of tool selection.} To assess the accuracy of the retrieval tool, we conducted experiments in four scenarios: (a) instructions not related to retrieving stickers. We randomly selected 1000 instruction data from BELLE's validation set, which can be considered unrelated to retrieving stickers. We calculate the percentage of instructions that do not contain the <ret> token as the accuracy rate. (b)-(e) Using retrieval instructions in both in-domain and out-of-domain training sets, with and without prefixes, i.e., the <pret> token. We consider the instructions involving in the training set as in-domain data. In (b)-(e), We random sample 1000 instruction in the test set of Sticker820k and calculate the percentage of replies containing the <ret> token as the accuracy rate.

\begin{table}[htbp]
\centering
\setlength\tabcolsep{3pt}
\begin{tabular}{lccccc} 
\toprule
Dataset   & BELLE      & Sticker    & Sticker    & Sticker    & Sticker     \\ \hline
In-domain & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55}  \\
Prefix    & \ding{55} & \ding{55} & \ding{55} & \ding{51} & \ding{51}  \\ 
Accuracy  & 96.7       & 68.1       & 53.6       & 100.0      & 100.0       \\
\bottomrule
\end{tabular}
\caption{Accuracy of tool selection in different settings.}
\label{tab:acc_tool_selection}
\end{table}

As shown in Tab. \ref{tab:sticker_clip_eval}, StickerLLM achieves an accuracy rate of 96.7\% on the BELLE test set. This indicates that for most instructions that are not related to sticker retrieval, StickerLLM doesn't executes the retrieval. Furthermore, since we completely freeze the model parameters (except for the embeddings in the positions of added special tokens), the StickerLLM model will yield identical responses as the original model when the special tokens are not generated. In (b)-(c), it is shown that the absence of prefixes does not alter the model's generation distribution, while the original language model is incapable of generating the <ret> token. Therefore, StickerLLM only uses the <ret> token for retrieval in sticker search instructions with a frequency of 68.1\% and 53.6\%, respectively. In (d)-(e), since we added the <pret> token as a prefix with a 50\% probability in the training data, the <pret> token has a stronger modulating ability for the subsequent retrieval tools. Therefore, StickerLLM can correctly invoke the retrieval tool, whether the sticker retrieval instructions are involved in the training data or not.

\textbf{Accuracy of Retrieval.} We also evaluated the accuracy of StickerLLM in retrieving stickers. During training, we constructed templates that unify text and image as input for retrieval instructions. Therefore, we report Recall@K (recall of the top K candidates) with K values of 1, 5, 10, and the Mean Recall (MR) for both image-to-image (I2I) and text-to-image (T2I) retrieval. In this experiment, we evaluated the retrieval performance of StickerLLM on the Emoji820K test set. 

\begin{table}[htbp]
\centering
\setlength\tabcolsep{3pt}
\begin{tabular}{ccccccc} 
\toprule
Method                      & Params                & Modality & R@1  & R@5  & R@10 & MR    \\ 
\hline
\multirow{2}{*}{StickerLLM} & \multirow{2}{*}{2.6M} & I2I      & 96.9 & 99.9 & 99.9 & 99.0  \\
                            &                       & T2I      & 61.5 & 82.4 & 87.5 & 77.1  \\
\bottomrule
\end{tabular}
\caption{Experimental results of StickerLLM in image-to-image (I2I) retrieval and text-to-image (T2I) retrieval.}
\label{tab:sticker_llm_eval}
\end{table}

As shown in Tab. \ref{tab:sticker_llm_eval}, the performance of StickerLLM to retrieve stickers based on images is much higher than its ability to retrieve stickers based on text (96.9\% R@1 image-to-image retrieval vs. 61.5\% text-to-image  
 retrieval). This is mainly because image features have richer and more specific semantic information compared to text features. Combining Table 1, when using ViT-B/16 as the image encoder, StickerLLM's performance on text-to-image retrieval exceeds the freeze-vision version based on ViT-B CLIP (77.1\% MR vs. 67.9\% MR), and is only surpassed by StickerCLIP ViT-B (77.1\% MR vs. 82.7\% MR). At the same time, StickerLLM's amount of trainable parameters is much lower than these two models, which demonstrates the potential for expanding the capabilities of LLM through prompt tuning.


\subsection{Qualitative Results}

\begin{figure}
\centering
\includegraphics[width=0.47\textwidth]{StickerCLIP_example.pdf}
\caption{Visualization results of StickerCLIP on Emoji820K.}
\label{fig:stickerclip_example}
\end{figure}

\textbf{Visualization of StickerCLIP.} We visualized the retrieval results of StickerCLIP and compared them with zero-shot retrieval results on the Emoji820k dataset, as shown in Figure 5. In this comparison, both our StickerCLIP and the Zero-shot model use the ViT-B structure, and we have shown the top 5 results of the same query retrieval. It can be seen that StickerCLIP performs better. For example, in the first example, the results of StickerCLIP can better express the state of confusion, in the second example, most of the results returned by the zero-shot model do not match the theme. in the third example, the Zero-shot model does not understand the meaning of "Rena Belle".


\begin{figure}
\centering
\includegraphics[width=0.47\textwidth]{StickerLLM_example.pdf}
\caption{Visualization results of StickerLLM on Emoji820K.}
\label{fig:stickerllm_example}
\end{figure}

\textbf{Visualization of StickerLLM.} StickerLLM accepts text queries and images as input, utilizes <ret> token to extract a unified retrieval embedding, which is aligned with the output features of visual encoder in StickerCLIP during the training process. In Fig. \ref{fig:stickerllm_example}, we present the visualization results of StickerLLM on the Emoji820K dataset, which can not only search stickers based on text queries alone, but also combine text and images for more refined retrieval. By randomly adding images as noise with a certain probability in the image-text instruction training data, StickerLLM can focus on text information rather than relying entirely on image information during joint image-text retrieval. The visual results of joint text and image retrieval by StickerLLM are shown in the third and fourth rows of Fig. \ref{fig:stickerllm_example}, where it can be observed that the search results of StickerLLM also meet the requirements of text queries when they are similar to the input images.


\begin{figure}
\centering
\includegraphics[width=0.47\textwidth]{StickerLLMvs.ChatGLMpdf.pdf}
\caption{Qualitative comparison between StickerLLM and ChatGLM-6B.}
\label{fig:stickerllm_vs_chatglm}
\end{figure}

\textbf{Performance of StickerLLM on common tasks.} We utilize ChatGLM-6B as the pretrained model of StickerLLM, freeze the model parameters and update only the embeddings corresponding to the positions of the newly added tokens. Thus it will not impact the performance of LLM on common tasks. In Fig. \ref{fig:stickerllm_vs_chatglm}, we showcase the responses of StickerLLM and ChatGLM on common instructions. It can be seen that the two models provide almost identical answers for the same instruction.
